An Open API Architecture to Discover the Trustworthy Explanation of Cloud AI Services

This article presents the design of an open-API-based explainable AI (XAI) service to provide feature contribution explanations for cloud AI services. Cloud AI services are widely used to develop domain-specific applications with precise learning metrics. However, the underlying cloud AI services remain opaque on how the model produces the prediction. We argue that XAI operations are accessible as open APIs to enable the consolidation of the XAI operations into the cloud AI services assessment. We propose a design using a microservice architecture that offers feature contribution explanations for cloud AI services without unfolding the network structure of the cloud models. We can also utilize this architecture to evaluate the model performance and XAI consistency metrics showing cloud AI services trustworthiness. We collect provenance data from operational pipelines to enable reproducibility within the XAI service. Furthermore, we present the discovery scenarios for the experimental tests regarding model performance and XAI consistency metrics for the leading cloud vision AI services. The results confirm that the architecture, based on open APIs, is cloud-agnostic. Additionally, data augmentations result in measurable improvements in XAI consistency metrics for cloud AI services.

==> Sections/section_n.tex <==

\subsection{Manuscript Setup}

The template is composed by a set of 7 files, in the
following 2 groups:\\
\noindent {\bf Group 1.} To format your paper you will need to copy
into your working directory, but NOT edit, the following 4 files:
\begin{verbatim}
  - apalike.bst
  - apalike.sty
  - article.cls
  - scitepress.sty
\end{verbatim}

\noindent {\bf Group 2.} Additionally, you may wish to copy and edit
the following 3 example files:
\begin{verbatim}
  - example.bib
  - example.tex
  - scitepress.eps
\end{verbatim}


\subsection{Page Setup}

The paper size must be set to A4 (210x297 mm). The document
margins must be the following:

\begin{itemize}
    \item Top: 3,3 cm;
    \item Bottom: 4,2 cm;
    \item Left: 2,6 cm;
    \item Right: 2,6 cm.
\end{itemize}

It is advisable to keep all the given values because any text or
material outside the aforementioned margins will not be printed.

\vfill
\subsection{First Section}

This section must be in one column.

\subsubsection{Title and Subtitle}

Use the command \textit{$\backslash$title} and follow the given structure in "example.tex". The title and subtitle must be with initial letters
capitalized (titlecased). The separation between the title and subtitle is done by adding a colon ":" just before the subtitle beginning. In the title or subtitle, words like "is", "or", "then", etc. should not be capitalized unless they are the first word of the title or subtitle. No formulas or special characters of any form or language are allowed in the title or subtitle.

\subsubsection{Authors and Affiliations}

Use the command \textit{$\backslash$author} and follow the given structure in "example.tex". Please note that the name of each author must start with its first name.

\subsubsection{Keywords}

Use the command \textit{$\backslash$keywords} and follow the given structure in "example.tex". Each paper must have at least one keyword. If more than one is specified, please use a comma as a separator. The sentence must end with a period.

\subsubsection{Abstract}

Use the command \textit{$\backslash$abstract} and follow the given structure in "example.tex".
Each paper must have an abstract up to 200 words. The sentence
must end with a period.

\subsection{Second Section}

Files "example.tex" and "example.bib" show how to create a paper
with a corresponding list of references.

This section must be in two columns.

Each column must be 7,5-centimeter wide with a column spacing
of 0,8-centimeter.

The section text must be set to 10-point.

Section, subsection and sub-subsection first paragraph should not
have the first line indent.

To remove the paragraph indentation (only necessary for the
sections), use the command \textit{$\backslash$noindent} before the
paragraph first word.

If you use other style files (.sty) you MUST include them in the
final manuscript zip file.

\vfill
\subsubsection{Section Titles}

The heading of a section title should be in all-capitals.

Example: \textit{$\backslash$section\{FIRST TITLE\}}

\subsubsection{Subsection Titles}

The heading of a subsection title must be with initial letters
capitalized (titlecased).

Words like "is", "or", "then", etc. should not be capitalized unless
they are the first word of the subsection title.

Example: \textit{$\backslash$subsection\{First Subtitle\}}

\subsubsection{Sub-Subsection Titles}

The heading of a sub subsection title should be with initial letters
capitalized (titlecased).

Words like "is", "or", "then", etc should not be capitalized unless
they are the first word of the sub subsection title.

Example: \textit{$\backslash$subsubsection\{First Subsubtitle\}}

\subsubsection{Tables}

Tables must appear inside the designated margins or they may span
the two columns.

Tables in two columns must be positioned at the top or bottom of the
page within the given margins. To span a table in two columns please add an asterisk (*) to the table \textit{begin} and \textit{end} command.

Example: \textit{$\backslash$begin\{table*\}}

\hspace*{1.5cm}\textit{$\backslash$end\{table*\}}\\

Tables should be centered and should always have a caption
positioned above it. The font size to use is 9-point. No bold or
italic font style should be used.

The final sentence of a caption should end with a period.

\begin{table}[h]
\caption{This caption has one line so it is
centered.}\label{tab:example1} \centering
\begin{tabular}{|c|c|}
  \hline
  Example column 1 & Example column 2 \\
  \hline
  Example text 1 & Example text 2 \\
  \hline
\end{tabular}
\end{table}

\begin{table}[h]
\vspace{-0.2cm}
\caption{This caption has more than one line so it has to be
justified.}\label{tab:example2} \centering
\begin{tabular}{|c|c|}
  \hline
  Example column 1 & Example column 2 \\
  \hline
  Example text 1 & Example text 2 \\
  \hline
\end{tabular}
\end{table}

Please note that the word "Table" is spelled out.

\vfill
\subsubsection{Figures}

Please produce your figures electronically, and integrate them into
your document and zip file.

Check that in line drawings, lines are not interrupted and have a
constant width. Grids and details within the figures must be clearly
readable and may not be written one on top of the other.

Figure resolution should be at least 300 dpi.

Figures must appear inside the designated margins or they may span
the two columns.

Figures in two columns must be positioned at the top or bottom of
the page within the given margins. To span a figure in two columns please add an asterisk (*) to the figure \textit{begin} and \textit{end} command.

Example: \textit{$\backslash$begin\{figure*\}}

\hspace*{1.5cm}\textit{$\backslash$end\{figure*\}}

Figures should be centered and should always have a caption
positioned under it. The font size to use is 9-point. No bold or
italic font style should be used.

\begin{figure}[!h]
  \centering
   {\epsfig{file = SCITEPRESS.eps, width = 5.5cm}}
  \caption{This caption has one line so it is centered.}
  \label{fig:example1}
 \end{figure}

\begin{figure}[!h]
  \vspace{-0.2cm}
  \centering
   {\epsfig{file = SCITEPRESS.eps, width = 5.5cm}}
  \caption{This caption has more than one line so it has to be justified.}
  \label{fig:example2}
  \vspace{-0.1cm}
\end{figure}

The final sentence of a caption should end with a period.



Please note that the word "Figure" is spelled out.

\subsubsection{Equations}

Equations should be placed on a separate line, numbered and
centered.\\The numbers accorded to equations should appear in
consecutive order inside each section or within the contribution,
with the number enclosed in brackets and justified to the right,
starting with the number 1.

Example:

\begin{equation}\label{eq1}
    a=b+c
\end{equation}

\subsubsection{Algorithms and Listings}

Algorithms and Listings captions should have font size 9-point, no bold or
italic font style should be used and the final sentence of a caption should end with a period.
Captions with one line should be centered and if it has more than one line it should be set to justified.

\vfill
\subsubsection{Program Code}\label{subsubsec:program_code}

Program listing or program commands in text should be set in
typewriter form such as Courier New.

Example of a Computer Program in Pascal:

\begin{small}
\begin{verbatim}
 Begin
     Writeln('Hello World!!');
 End.
\end{verbatim}
\end{small}


The text must be aligned to the left and in 9-point type.

\subsubsection{Reference Text and Citations}

References and citations should follow the APA (Author, date)
System Convention (see the References section in the compiled
manuscript). As example you may consider the citation
\cite{Smith98}. Besides that, all references should be cited in the
text. No numbers with or without brackets should be used to list the
references.

References should be set to 9-point. Citations should be 10-point
font size.

You may check the structure of "example.bib" before constructing the
references.

For more instructions about the references and citations usage
please see the appropriate link at the conference website.

\section{\uppercase{Copyright Form}}

For the mutual benefit and protection of Authors and
Publishers, it is necessary that Authors provide formal written
Consent to Publish and Transfer of Copyright before publication of
the Book. The signed Consent ensures that the publisher has the
Author's authorization to publish the Contribution.

The copyright form is located on the authors' reserved area.

The form should be completed and signed by one author on
behalf of all the other authors.

\section{\uppercase{Conclusions}}
\label{sec:conclusion}

Please note that ONLY the files required to compile your paper should be submitted. Previous versions or examples MUST be removed from the compilation directory before submission.

We hope you find the information in this template useful in the preparation of your submission.

\vfill
\section*{\uppercase{Acknowledgements}}

If any, should be placed before the references section
without numbering. To do so please use the following command:
\textit{$\backslash$section*\{ACKNOWLEDGEMENTS\}}

\section*{\uppercase{Appendix}}

If any, the appendix should appear directly after the
references without numbering, and not on a new page. To do so please use the following command:
\textit{$\backslash$section*\{APPENDIX\}}

==> Sections/section_n1.tex <==
\section{\uppercase{Evaluation with interviews}}
\label{sec:interview}
An interview with the demos followed by conversations on six questions serves as the preliminary user-based evaluation.
Ten participants, including eight machine learning engineers and two cloud service architects, are invited for the interview.
Based on the interview responses, the overall impression of the XAI service system is positive. 

\begin{figure}[htbp]
\centerline{\includegraphics[width=6.5cm]{Charts/interviewplot.png}}
\caption{A summarized interview feedback for the XAI service}
\label{interview}
\end{figure}

For knowledge of XAI techniques, three out of ten participants knew the concept of XAI but had no previous experience using an XAI service or other approach. 
By reviewing the demonstration of the system, nine of ten participants could understand the image explanations provided by the XAI service system. 
The system is generally considered easy to understand, but three participants have suggested providing instructions or tutorials for non-AI-experts users. 
All participants agree that the provenance data can provide transparency in XAI operations, trace past actions and reproduce the results of others. The provenance data is a valuable resource for the user. 
Participants have also suggested additional features to be added to the XAI service system, such as visualization of the service architecture and data pre-processing. 
One participant also raised the need for an A/B testing mechanism with a feedback section in the system, which could be helpful in testing and improving the system's performance over time. 
The interview feedback is summarized in Figure \ref{interview}.

Additionally, some participants would like to see more XAI cases in the XAI service system. Currently, we provide three models and five XAI methods with evaluation metrics. In the future, more state-of-the-art XAI techniques and external AI models can be integrated into the system. 

==> Sections/section_n2.tex <==
\section{\uppercase{The Technical Soundness Discussions}}
\label{sec:Discussions}

\subsection{Reusability of the Microservices}
Reusability is one of the advantages of using microservices architecture in XAI systems.
We present the design of four types of microservices, including data processing, AI model, XAI method and evaluation. Every kind of microservice is designed for a specific type of role in XAI operations. The APIs are also unified for the specific duty. Therefore, the XAI service can be flexibly reused with different microservices.
For example, the ResNet model, integrated into the AI model microservice, is responsible for taking images as input and computing predictions as output. 
By replacing a new AI model microservice with a unified API, such as the DenseNet model microservice. The other role of microservice can still be used to execute the XAI pipelines. 
By following this design, the new microservice can integrate with the XAI service without changes to the other parts.
The independent development of microservice allows for flexibility in the application of state-of-the-art AI models and XAI methods.

% By deploying well-developed microservices, users can improve the performance of the XAI service and reduce development costs. For instance, state-of-the-art AI models such as ResNet50 can be commonly used and reused across different scenarios \cite{huq2022application}. Additionally, XAI methods can also be reusable. CAM-based methods can be applied to various convolutional neural network (CNN) models, such as ResNet and DenseNet, shown in Section \ref{sec:casestudies}. Furthermore, some unified XAI methods can be applied to a wide range \cite{lundberg2017unified}. This reusability allowing developers to focus on XAI tasks application rather than dedicating efforts to engineering a whole platform.

\subsection{The Effort for Developing the Added Microservice}

\subsubsection{Lines of Code (LoC)}

We count the lines of code for the microservices in Table ~\ref{loc}, specifically, the number before and after integrating the model or algorithm into the microservice.

\begin{table}[htbp]
\caption{Lines of Code statistic of turning the existing code to microservice application}
\renewcommand{\arraystretch}{1.2}
\begin{center}
\begin{tabular}{M{1.6cm} | M{1.3cm} M{1cm} M{1.4cm} M{1.2cm}}
\hline
\textbf{}&\multicolumn{4}{c}{\textbf{XAI Component}} \\
\textbf{LoC before and after Microservice} & \textbf{\textit{Azure Cognitive Service}} &  \textbf{\textit{ResNet50 Model}} &  \textbf{\textit{Grad-CAM Method}} &  \textbf{\textit{Evaluation}} \\ 
\hline
before   &   128 &     56 &    192 &    372 \\
after   &   156 (+28) &     98 (+42) &   248 (+56) &    453 (+81) \\

\hline
\end{tabular}
\label{loc}
\end{center}
\end{table}
 
\subsubsection{Steps for Building the Existing Code into a Microservice}

To transfer the existing code to the microservice, we take the following steps:
\begin{itemize}
    \item[1.] Build an HTTP server base;
    \item[2.] Embed the existing code into the server base as a function module;
    \item[3.] Follow the convention, convert the input of the HTTP request into the model or the function;
    \item[4.] Follow the convention, convert the output of the model or the function into the HTTP response, and upload the operation result to the database;
\end{itemize}

%The convention of the service input and output should be made by the platform that connects all XAI components together to ensure the components correctly communicate with each other.

\subsection{Carbon Footprint of the XAI Tasks}
In addition to the stability and consistency evaluation metrics, shown in Figure \ref{stability_cam}-\ref{dens_consistency_cam}, two metrics are collected for the XAI operations shown in Figure \ref{carbon}. Namely, the power consumption and carbon emissions estimation of the executed tasks. 
\begin{figure}[ht]
\centerline{\includegraphics[width=\linewidth]{Charts/carbon}}
\caption{Energy consumption and carbon emissions example for a task run, shown by a screenshot from the user interface}
\label{carbon}
\end{figure}
The metrics provide another view of the microservices' performance and enable users to make more informed decisions about the deployment and use of XAI and work towards reducing their overall environmental impact.

==> Sections/section_x4.tex <==
\section{\uppercase{XAI Service Architecture and API Design}}
\label{sec:Design}
\noindent
Since the RESTful APIs are the entry to access a cloud-based AI service, the integration of involved components and operations in Figure \ref{flow-chart} represent the form of services using APIs defined on the service endpoints. This is one key factor in proposing the design of microservices for XAI operations. 

The design of XAI operations as microservices leads us to define a reference architecture that consists of four layers, the user interface layer, the coordination center layer, the core microservice layer, and the data persistence layer. The overview of the reference architecture is shown in Figure \ref{architecture}.

\begin{figure*}[ht]
\centerline{\includegraphics[width=\linewidth]{Charts/APIarchetecture-Page-2.drawio.png}}
\caption{Reference architecture design for XAI service in a microservice-based approach}
\label{architecture}
\end{figure*}

One key feature of this proposed architecture is its non-intrusive application of XAI methods. This approach allows us to apply XAI techniques without significantly disrupting or modifying existing system operations. We have completed the API design for this microservice system, with these APIs systematically arranged and hosted on Swagger Hub, adhering to OpenAPI 3.0 specifications. Figure \ref{swaggerapi} offers a snapshot of the API documentation, featuring an array of functional interfaces. We delve into the specific functionalities of these APIs in the following subsections.

\begin{figure}[ht]
\centerline{\includegraphics[width=\linewidth]{Charts/swaggerAPI.png}}
\caption{Snapshot of the organized APIs in the XAI service documentation}
\label{swaggerapi}
\end{figure}


\subsection{User Interface}
\noindent
The user interface allows users to set a task or combine tasks into a pipeline. To perform an XAI task, users fill in various microservices' service addresses and configurations to set up the task. Then, users fill in parameters for the task to be executed, such as the corresponding data set and XAI method settings. 

The user interface supports three forms: Web portal, RESTful APIs, and command line to view and send operations to invoke the XAI microservices. The user interface provides multiple components, including microservice registration, XAI task configuration, explanation summary, and provenance data plotting in a graph view. To assist developers in generating new XAI services and managing pipelines, the user interface layer exposes RESTful APIs, thereby facilitating the transmission of requests to and receipt of responses from the coordination center.


%This layer ensures that the coordination center captures all operation history and enables the XAI data provenance feature.
%To interact with the coordination center, we should first have the deployed back-end server of the coordination center then we can interact with it.


%The layer also releases the front-end application, which leverages the RESTful API and provides more user interaction and visual experience for the XAI service. 
% The user interface allows users to set a task or wire them to a pipeline. 
% To perform an XAI task, users need to fill in the addresses and types of various microservices to set up the task. 
% Then, users also need to fill in parameters for the task to be executed, such as the corresponding dataset and XAI method parameters. 
% Users can execute the task by commands on the user interface.


\subsection{Coordination Center}
\noindent
The coordination center incorporates the server that processes requests from the user interface layer and activates the corresponding components for operation completion. The primary functionalities are microservice management, XAI operation management, and data representation.

In microservice management, the coordination center receives information from the user interface regarding microservices registration and modification. The microservices endpoints and functional types are documented in this layer. When a user executes an XAI task, the coordination center retrieves the corresponding microservice.

Under the XAI operation management, the coordination center allows users to edit a task sheet which keeps the information about the task type (XAI task or evaluation task), the involved services, the data set, and the task execution parameters. 
Furthermore, the Coordination Center administers the lifecycle of the task execution. The task execution follows the task sheet. It is a runtime sub-process that takes the information from the task sheet, inquires about the data, invokes APIs from the involved services, and executes the task.
Once the executor executes the task, it sends the task status (succeed or failed) and the runtime information (carbon emission and energy consumption estimation) back to the coordination center. 
The coordination center also provides pipeline configuration, which consists of one XAI task sheet and one evaluation task sheet. 
The purpose of the pipeline is to execute the XAI task followed by the evaluation task serially.
Accordingly, the coordination center controls the live cycle of the pipeline execution, which is similar to the task execution.

The data representation component retrieves information from the data persistence layer and presents various sources for the user to understand the explanation conclusion, such as XAI summaries, evaluation metrics, and provenance data for historical views.

% When the user wants to execute a task from a task sheet, the model creates a task instance from the task sheet with a unique task ticket and then sends all task configurations to the executor.
% The user can execute a task from a task sheet through the coordination center.
% When the executor finishes the task process or an error occurs, the executor will send the task status (finished or error) to the coordination center. 
% The user can also stop the task through the coordination center in the middle.
% The pipeline is a configuration that combines the XAI task sheet and the evaluation task sheet and executes tasks from them one by one.
% The pipeline run is the running instance of the pipeline. The system also provides the life cycle control for the pipeline run.

% The data presentation division retrieves information from the data persistence layer and presents the XAI results, evaluation results, and provenance data to the user interface. This division allows for easy access and understanding of the results.

\subsection{Microservice Layer}
\noindent
The diversities of data set persistence, AI models, XAI methods, and evaluation metrics form a large and complex space to define the connections among these entities. Encapsulating these entities into microservices significantly reduces the microservices into four kinds, as follows. This converts the complicated heterogeneous components integration problem into the clear operations of connecting these services through open APIs with endpoints.

\subsubsection{The Data Processing Microservice}
\noindent
%One of the key purposes of XAI is to evaluate the generalizability and consistency of a trained model. To do this effectively, 
%The data used for testing the model must accurately represent real-world contexts.
In our system, XAI operations are premised on the assumption that test datasets have been preprocessed and are prediction-ready. Users upload raw, labeled data to the database, structuring datasets suitable for XAI operation. In our reference architecture, accessing these datasets is considered an operation in line with other XAI operations.


\subsubsection{The AI Model Microservice}
\noindent
% Interacting with the AI model is required by either model-specific or model-agnostic XAI methods.
% Model-specific XAI methods require access to the content inside a model, such as the model's internal structure and parameters. This allows the XAI method to provide explanations tailored to the specific model.
% On the other hand, model-agnostic XAI methods can provide explanations through the input and output of the model without requiring access to the model's internal content. These methods treat the model as a black box and calculate the feature attribution values by obtaining the output for controlled specific input.
% To facilitate XAI service, the AI model can be integrated as a microservice, which enables the XAI system to access the model and use it to provide explanations.
% In addition, using pre-trained models as microservices require less computational resource and provide a default selection of models for the common user application scenarios. We have deployed pre-trained models for computer vision test cases demonstrative of usage scenarios.
An AI model microservice encapsulates a pretrained deep learning model with a designated endpoint. Architecturally, predictions are invoked on AI models similarly to cloud-based AI services, executed through the sending and receiving of HTTP requests from the open service APIs.

The architecture design encapsulates AI models and XAI methods as microservices and enables the post hoc explanation based on the feature influence depicted in Figure~\ref{flow-chart}. In this paper, we deploy and register two state-of-the-art pre-trained deep learning models as microservices. Hence, the learning model of cloud-based AI microservice can be approximated by deep learning model services. 


%Additionally, some model-specific XAI methods require access to the model's structure and parameters. 
%Hence the AI model microservice can also provide the option to access the model's parameters.


\subsubsection{The XAI Method Microservice}
\noindent
XAI method microservice refers to the deployment of XAI methods as microservices.  
The XAI method microservices support both model-specific and model-agnostic methods. These methods provide explanations based on feature contribution values.  
It allows access to data processing microservice and AI model microservice through RESTful API and can provide explanations. 
%We use the systematic selection of the XAI techniques based on the study~\cite{Anonymous-1}.

%For example, Grad-CAM\cite{selvaraju2017grad} can provide explanations for many Convolutional Neural Network models such as ResNet and DenseNet\cite{resnet,huang2017densely}.

\subsubsection{The Evaluation Microservice}
\noindent
Evaluation of the XAI method guides AI practitioners to choose and trust models and XAI methods. The evaluation microservice can provide functionalities to evaluate the model's and XAI's performance by analyzing the explanation results. The service employ the XAI consistency evaluation \cite{paper1}

% Our previous work has discovered that XAI methods produce an explanation in variation~\cite{paper1,paper2}. We define explanation stability to refer to the explanation variation of one XAI method on different data samples. We further define explanation consistency as the explanation variation among multiple XAI methods on the same data samples. As shown in Figure~\ref{flow-chart}, the evaluation service concludes the XAI pipeline and provides AI practitioners with cross-validated explanation summaries. 


%Evaluation of the XAI method guides AI practitioners to choose and trust models and XAI methods. The evaluation microservice can provide functionalities to evaluate the performance of the model and XAI by analyzing the explanation results. 
%Fewer studies deliver a consensus standard as an evaluation metric. We develop the stability evaluation metrics~\cite{Anonymous-1} in the microservice, which can calculate the defined distance value between the data samples and summarize a stability value. The definition is specified in section \ref{sec:casestudies} equation \ref{eq:stability}.



\subsection{Data Persistence Layer}
\noindent
The data persistence layer manages the queries and storage of data sets, XAI operation data, explanation summaries, and evaluation results. The design of XAI provenance metadata is further introduced in section \ref{sec:provenance}. 
%The case studies have explanation results and evaluation results in illustration in section \ref{sec:casestudies}.

Overall, the reference architecture considers the microservice the unified deployment form regardless of the XAI operation types, variety of AI models, AI services, and XAI methods. Users have the flexibility to select microservices.



==> Sections/section_x6.tex <==
\section{\uppercase{Experiment Setup and XAI Service Configuration}}
\label{sec:Configuration}
\noindent

{\color{blue}\subsection{Objective of the Experiments}
The experiments are to validate the applicability and efficiency of the microservices-based architecture. We demonstrate how our system integrates various pre-trained AI models and cloud-based AI services through a series of experiments. And we employ state-of-the-art CAM-based computer vision XAI techniques for the cloud AI models.

The experiments are designed to answer the following key questions:

\begin{itemize}
\item What metrics can demonstrate the XAI service's capability to integrate and utilize various cloud AI models and XAI methods?
\item When assessing the performance of cloud AI and XAI methods, how do the computed result of prediction change values and stability evaluations?
\item Based on the results, what specific factors influence the performance and stability of XAI methods, and how can these factors be optimized for more reliable explanations?
%\item Can the system work on different cloud platforms such as Azure Cognitive Service, Google Vertex AI, and Amazon Rekognition?
\end{itemize}

By addressing these questions, the experiments seek to validate the design of our XAI service system and assess its performance in real-world scenarios.
}





%%%%%%%%%%%%%%%%%%ENd%%%%%%%%%%%%%%%%
% After the configuration of the XAI and evaluation task sheets, they are sequenced into two pipelines for efficient execution. The outcome of these pipelines is analyzed and visualized, providing a detailed understanding of the model's performance, thus contributing to the field of explainable artificial intelligence.


%This section provides the experimental configuration, including the design and execution of the evaluation metrics for the XAI services. 
%The microservices are registered within the coordination center and span across distinct domains, as depicted in Figure \ref{architecture}.
% These microservices are either directly incorporated into the XAI service or are customized to align with user-specific requirements. This flexible architecture allows for the seamless integration of external resources as microservices, highlighting the adaptable nature of the XAI service.

% In this section, we elaborate on the design of experimental operations. 
% Our experimental setup utilizes the ImageNet dataset\cite{deng2009imagenet}. The dataset feeds into a database microservice, which is responsible for storing and managing the data for subsequent testing.

% We develop an AI microservice, integrating the cloud AI service using a Restful API. Alongside this, the XAI microservices are equipped to implement CAM-based methods for generating saliency map explanations.

% The orchestration of these microservices is handled by the coordination center. This allows for the execution of explanation tasks via API calls, leading to the production of saliency maps. The overall system design ensures an efficient workflow for the generation of explanations.

%This multifaceted microservices approach underscores the versatility and adaptability of our experimental design.
% We configure two XAI task sheets: (1) use the ResNet model to generate the explanation; (2) use the DenseNet model to generate the explanation.
% Inside the XAI task, the XAI method microservice is the task executor. The XAI executor retrieves the test set from the Azure Blob database microservice, downloads the model's parameters from the approximation AI model, and executes the XAI method.
% We also configure two evaluation task sheets using the Azure Cognitive Service microservice to evaluate the explanations from the above two XAI tasks.
% The objective of the evaluation tasks is to determine whether the explanations generated by the two approximation models, ResNet and DenseNet, are also applicable as explanations for the Cloud AI Services model.
% In the context of the evaluation task, both original and masked images are supplied to the Cloud AI Services, resulting in prediction change values. The evaluation microservice performs operations outlined in Figure \ref{flow-chart}.
% These prediction change values are then consolidated into the unified consistency metric~\cite{paper1}, which aids in analyzing the overall effectiveness and performance of the XAI method. 

% After the two XAI task sheets and two evaluation task sheets are configured, we assemble them into two pipelines for serial task execution. 

% Once we get the stability and consistency metrics from the two pipelines running results, the distribution of prediction changes and probability density of the distance values can be plotted and visualized. 
% Stability metrics are a type of statistical evaluation that uses a fixed data set to assess the results of XAI methods. 
% Additionally, by selecting the method that has the best stability performance as a baseline, we can further evaluate the consistency by comparing it with other methods. 


% %\subsection{Design of the Experimental Operations}
% We have conducted a thorough assessment of the results from our XAI service, with a central goal to illuminate the explanations generated by our cloud AI service. This section emphasizes evaluating the consistency of our XAI service's explanations, followed by an examination of the operational overhead it entails.

